The environment as a driver of galaxy evolution with the miniJPAS survey

This thesis aims at discerning the effect of environment on galaxy evolution and on the properties of galaxies, using the data from the miniJPAS survey, a 1~deg$^2$ survey that uses the same photometric filter system as the incoming J-PAS survey, which is already in its scientific verification phase. This system is composed of 56 narrow-band filters that provide an spectral resolution comparable to low-resolution spectroscopy. We study the effect of environment using two approaches. First, we study the spatially resolved galaxies from miniJPAS. Secondly, we studied the galaxy population in the most massive galaxy cluster detected in the miniJPAS footprint, that is, the cluster mJPC2470-1771. We have developed a tool that automatises all the required processes for the analysis of the data. After probing the accuracy and reliability of the photmetry obtained with our tool, we apply it to a miniJPAS sample of spatially resolved galaxies, divided into four sub-samples according to their spectral-type (red/quiescent and blue/star forming), and environment (field or galaxy group). We find that redder, denser regions are usually older, more metal rich, and show lower values of the intensity of the star formation rate and the specific star formation rate than bluer and less dense regions. Regarding the mJPC2470-1771 cluster, our results point that more massive, redder and older galaxies typically populate the inner regions of the cluster. As a conclusion, our results suggest that galaxies in clusters are formed at a similar epoch, but have experienced different star formation histories. We conclude that the environment plays a role on galaxy evolution, but it is mainly reflected through the galaxy populations found in high density environments, such as galaxy clusters and groups, where the fraction of red, quiescent galaxies is larger in comparison to the field.

==> declaration/declaration.tex <==
\begin{center}
\thispagestyle{empty}
%{\textbf{\textit{SYNOPSIS OF}}}
\vskip .5cm
{\centerline {{\textbf{DECLARATION}}}}
\end{center}

% {\Large \textbf {An Overview}}
% \vskip .2cm
% {\Large \textbf {of}}
% \vskip .2cm
% {\Large \textbf {Everything}}
\par \quad \quad I here by declare that the thesis entitled \enquote{Thesis Title} submitted by me, for the award of the degree of {\it Doctor of Philosophy} to VIT University is a record of bonafide work carried out by me under the supervision of Dr. Guide Name, Designation, School or Centre Name, VIT University, Vellore.
\vskip 0.5cm
\noindent
\par \qquad
I further declare that the work reported in this thesis has not been submitted
and will not be submitted, either in part or in full, for the award of any other degree or
diploma in this institute or any other institute or university.
~\\
~\\
~\\
~\\
~\\
~\\
~\\
\noindent
Place: Vellore
\vskip 0.3cm
\noindent
Date:     \qquad \qquad \qquad \qquad  \qquad \qquad \qquad \qquad \qquad \quad \quad          						 \textbf{Signature of the Candidate}

==> preamble/acronyms.tex <==
\chapter*{List of Terms and Abbreviations}
\addcontentsline{toc}{chapter}{List of Terms and Abbreviations}
\begin{acronym}[TDMA]
    \acro{ADQL}{Astronomical Data Query Language}
    \acro{ADU}{Astronomical Digital Unit}
    \acro{AGN}{Active Galactic Nuclei}
    \acro{ALHAMBRA}{Advance Large Homogeneous Area Medium Band Redshift Astronomical}
    \acro{AMICO}{Adaptive Matched Identifier of Clustered Objects}
    \acro{ANN}{Artificial Neural Network}
	\acro{API}{Application Programming Interface}
    \acro{\texttt{BatMAN}}{Bayesian Technique for Multi-image Analysis}
    \acro{CALIFA}{Calar Alto Legacy Integral Field Area}
    \acro{CCD}{charge-coupled device}
    \acro{COMBO-17}{Classifying Objects by Medium-Band Observations}
    \acro{COSMOS}{Cosmic Evolution Survey}
    \acro{DES}{Dark Energy Survey}
    \acro{ELG}{Emission Line Galaxy}
    \acro{EW}{Equivalent Width}
    \acro{FoV}{Field of View}
    \acro{GEMS}{Galaxy Evolution from Morphology and SEDS}
    \acro{HLR}{Half-light radius}
    \acro{HMR}{Half-mass radius}
    \acro{HSC-SSP}{Hyper Suprime-Cam Subaru Strategic Program}
    \acro{IFS}{Integral Field Spectroscopy}
    \acro{IFU}{Integral Field Unit}
    \acro{ICM}{Intra Cluster Medium}
    \acro{IGM}{Inter Galactic Medium}
    \acro{IMF}{IMF}{Initial Mass Function}
    \acro{ISM}{Inter Stellar Medium}
    \acro{HMR}{Half Mass Radius}
    \acro{HLR}{Half Light Radius}
    \acro{FWHM}{Full Width Half Maximum}
    \acro{J-PAS}{Javalambre-Physics of the Accelerated Universe Astrophysical Survey}
    \acro{JPAS-PF}{J-PAS Pathfinder}
    \acro{JPCam}{Javalambre Panoramic Camera}
    \acro{J-PLUS}{Javalambre Photometric Local Universe Survey}
    \acro{MaNGA}{Mapping Nearby Galaxies at Apache Point Observatory}
    \acro{MCMC}{Markov Chain Monte Carlo}
    \acro{OAJ}{Observatorio Astofísico de Javalambre}
    \acro{Pan-STARRS1}{ Panoramic Survey Telescope and Rapid Response System 1}
    \acro{PMAS}{Potsdam Multi Aperture Spectrograph}
    \acro{PDF}{Probability density function}
    \acro{PSF}{Point Spread Function}
    \acro{QFE}{Quenched Fraction Excess}
    \acro{QSO}{Quasi Stellar Object}
    \acro{ReLU}{Rectified Linear Unit}
    \acro{SAURON}{Spectroscopic Areal Unit for Research on Optical Nebulae} 
    \acro{SDSS}{Sloan Digital Sky Survey}
    \acro{SED}{Spectral Energy Distribution}
    \acro{SFMS}{Star Formation Main Sequence}
    \acro{SFH}{Star Formation History}
    \acro{SFR}{Star Formation Rate}
    \acro{S-PLUS}{Southern Photometric Local Universe Survey}
    \acro{sSFR}{Specific Star Formation Rate}
    \acro{SSP}{Single Stellar Population}
    \acro{TAP}{Table Access Protocol}
    \acro{UPAD}{Unidad de Procesado y Archivo de Datos}
    \acro{VIPERS}{VIMOS Public Extragalactic Redshift Survey}
    \acro{VO}{Virtual Observatory}
    \acro{VUDS}{VIMOS Ultra Deep Survey}
    \acro{VVDS}{VIMOS VLT Deep Survey}
    \acro{WCS}{World Coordinate System}
    \acro{ZP}{Zero Point} 
    \acro{$z\mathrm{PDF}$}{Probability density function of the redshift}
      
\end{acronym}

==> publications.tex <==
\chapter*{\centering \large\textbf{LIST OF PUBLICATIONS}}
\addcontentsline{toc}{section}{\bf ~~~~~~~~~~~LIST OF PUBLICATIONS}
\noindent
\begin{enumerate}
	\item Anouncia, S.M. and Saravanan, R., 2006. Non-destructive testing using radiographic images a survey. Insight-Non-Destructive Testing and Condition Monitoring, 48(10), pp.592-597.
	
	\item Amalanathan, A. and Anouncia, S.M., 2016. A review on user influence ranking factors in social networks. International Journal of Web Based Communities, 12(1), pp.74-83.	
\end{enumerate}
